Online Real-time Multiple Spatiotemporal Action Localisation and Prediction

We present a deep-learning framework for real-time multiple spatio-temporal (S/T) action localisation, classification and early prediction. Current state-of-the-art approaches work offline and are too slow to be useful in real- world settings. To overcome their limitations we introduce two major developments. Firstly, we adopt real-time SSD (Single Shot MultiBox Detector) convolutional neural networks to regress and classify detection boxes in each video frame potentially containing an action of interest. Secondly, we design an original and efficient online algorithm to incrementally construct and label `action tubes' from the SSD frame level detections. As a result, our system is not only capable of performing S/T detection in real time, but can also perform early action prediction in an online fashion. We achieve new state-of-the-art results in both S/T action localisation and early action prediction on the challenging UCF101-24 and J-HMDB-21 benchmarks, even when compared to the top offline competitors. To the best of our knowledge, ours is the first real-time (up to 40fps) system able to perform online S/T action localisation and early action prediction on the untrimmed videos of UCF101-24.

==> text/soa_bmvc.tex <==
\section{Related work}

\iffalse
%----------------action classification---------------------
Many approaches to action recognition \cite{laptev-2008,wang-2011,wang-2013} are based on appearance 
(e.g. HOG \cite{dalal-2005}, SIFT \cite{Lowe-2004}) or motion features 
(e.g., optical flow, MBH \cite{dalal-2006}),
encoded using Bag of Visual Words \cite{csurka2004visual} or Fisher vectors \cite{perronnin2007fisher}
The resulting descriptors are typically used to train classifiers (e.g. SVM) in order to predict the labels of action videos.
\fi

%-----------------cnn based action classification and localisation--------------------
Recently, inspired by the record-breaking performance of CNNs in image classification \cite{krizhevsky2012} 
and object detection from images \cite{girshick-2014},
deep learning architectures have been increasingly applied to action classification \cite{Shuiwang-2013,Karpathy-2014,Simonyan-2014}, 
spatial \cite{Georgia-2015a} or spatio-temporal 
\cite{Weinzaepfel-2015} action localisation,  
and event detection \cite{xu2014discriminative}. 
\iffalse %Repetition.
Indeed %, inspired by this success %of \cite{Georgia-2015a} and \cite{Simonyan-2014}, 
we also extract CNN features, both from RGB and optical flow-derived motion images,
but instead of concatenating the features and passing them to a classifier,
we perform region proposal and detection simultaneously using \emph{a single Faster-RCNN network, trained end-to-end,
and then merge the results using a score compatibility function}.
\fi
% localisation (spatial or spatio-temporal)

The %\textbf{action localisation} 
action localisation problem, in particular, can be addressed by leveraging on video segmentation methods.
An example is the unsupervised greedy agglomerative clustering approach of \cite{jain2014tublet}, which resembles Selective Search space-time video blocks.
Since \cite{jain2014tublet} does not exploit the representative power of CNN features, they fail to achieve state-of-the-art results.
Soomro~\etal~\cite{Soomro2015} learn the contextual 
relations between different space-time video segments. Such `supervoxels', however, may end up spanning very long time intervals, failing to localise each action instance individually.
Similarly, \cite{vanGemert2015apt} uses unsupervised clustering to generate a small set of bounding box-like spatio-temporal action proposals.
%Although the authors rely on the branch-and-bound search algorithm \cite{yuan2011discriminative}, %with the addition of motion trajectories, 
However, since the approach in \cite{vanGemert2015apt} employs dense-trajectory features 
%which rely on motion 
\cite{wang-2011},
it does not work on actions characterised by small motions \cite{vanGemert2015apt}.

% context (also to improve localisation)
\iffalse
\textbf{Contextual cues} can be used to improve on action recognition and localisation. 
Whereas \cite{Georgia-2015b} is limited to localisation in still images,
\cite{Jain-2015} will only reap benefits where the objects involved in the action are discriminative.
By contrast, \emph{our method is data-driven and can discriminate between distinct actions categories involving the same objects}
(e.g. the `door' in LIRIS-HARL's `unsuccessfully unlocking door' and `successfully unlocking door' classes).
\fi

% temporal localisation
The %\textbf{temporal detection}
temporal detection of actions~\cite{jiang2014thumos,gorban2015thumos} 
and gestures~\cite{escalera2014chalearn} in temporally untrimmed videos has also recently attracted much interest \cite{yeung2015every,Evangel-2014}.
%These challenges led to big advances in the state-of-the-art \cite{yeung2015every}.
Sliding window approaches have been extensively used \cite{laptev2007retrieving,gaidon2013temporal,tian2013spatiotemporal,wang2014video}. 
%On the contrary, Evangelidis \etal \cite{Evangel-2014} show efficiency for dynamic programming for temporal trimming. 
%For instance, Tian et al. \cite{tian2013spatiotemporal} extend deformable part models to 3D and employed a sliding window which varied in scale, space and time.
%Wang \etal  \cite{wang2014video} first used a temporal sliding window and then modelled the relations between dynamic-poselets. 
Unlike our approach, these methods \cite{tian2013spatiotemporal,wang2014video,yeung2015every} only address \emph{temporal} detection,
and suffer from the inefficient nature of temporal sliding windows.
Our framework is based on incrementally linking frame-level region proposals and temporal smoothing (in a similar fashion to \cite{Evangel-2014}), 
{an approach which is computationally more efficient and can handle long untrimmed videos}. 


% spatio-temporal localisation via linking region proposals
Indeed %\textbf{methods which connect frame-level region proposals} 
methods which connect frame-level region proposals for joint spatial and temporal localisation
%(for instance using a human detector to generate bounding box region proposals \cite{yu2015fast})
have risen to the forefront of current research.
% our main competitors
%As clearly stated in the Introduction,
%we identify \cite{Georgia-2015a} and \cite{Weinzaepfel-2015} as our main competitors.
Gkioxari and Malik \cite{Georgia-2015a} have extended \cite{girshick-2014} 
and \cite{Simonyan-2014} to tackle action detection
%simultaneous action classification and localisation,
using unsupervised Selective-Search region proposals and separately trained SVMs.
However, as the videos used to evaluate their work only contain one action and were already temporally trimmed (J-HMDB-21~\cite{J-HMDB-Jhuang-2013}),
it is not possible to asses their temporal localisation performance.  
Weinzaepfel \emph{et al.}'s approach \cite{Weinzaepfel-2015}, instead, first generates region proposals using EdgeBoxes \cite{zitnick2014edge} at frame level to later 
use a tracking-by-detection approach based on a novel track-level descriptor called a Spatio-Temporal Motion Histogram. % Fabio: to do what? construct action paths/tubes?
Moreover, \cite{Weinzaepfel-2015} achieves temporal trimming using a multi-scale sliding window over each track, making it inefficient for longer video sequences.
Our approach improves on both \cite{Georgia-2015a,Weinzaepfel-2015} by using an efficient two-stage single network for detection of region proposals  
and two passes of dynamic programming for tube construction.

\iffalse
In opposition \emph{our approach is more efficient, as we use no intermediate representation and solve the linking problem efficiently via dynamic programming}.
This is shown in the results of Table \ref{table:speed}.
\fi

% include this paper in SOA- End-to-end Learning of Action Detection from Frame Glimpses in Videos

%\textbf{Multiple action detection}.
Some of the reviewed approaches \cite{Weinzaepfel-2015,vanGemert2015apt} could potentially be able to detect co-occurring actions.
However, \cite{Weinzaepfel-2015} {limit their method to produce maximum of two detections per class}, 
while \cite{vanGemert2015apt} does so on the MSRII dataset \cite{MSRIIcao2010cross} 
which only contains three action classes of repetitive nature (clapping, boxing and waving).
Klaser at al. \cite{klaser-2010} use a space-time descriptor and a sliding window classifier to detect the location of only two actions (phoning and standing up).
{In contrast, in our LIRIS-HARL tests (\S~\ref{sec:results_liris}) we consider 10 diverse action categories}.

\iffalse
In \cite{yeung2015every} a Long Short Term Memory network is proposed  
for multiple co-occurring action detection, %Fabio: sounds like we should say more on this paper
but spatial localisation is ignored.
\fi

%-  MAYBE A TABLE COMPARING OUR FEATURES TO THOSE OF MAIN COMPETITORS COULD BE GOOD TO PUT

